A Marriage between Adversarial Team Games and 2-player Games: Enabling Abstractions, No-regret Learning, and Subgame Solving

\emph{Ex ante} correlation is becoming the mainstream approach for \emph{sequential adversarial team games}, where a team of players faces another team in a zero-sum game. It is known that team members' asymmetric information makes both equilibrium computation \textsf{APX}-hard and team's strategies not directly representable on the game tree. This latter issue prevents the adoption of successful tools for huge 2-player zero-sum games such as, \emph{e.g.}, abstractions, no-regret learning, and subgame solving. This work shows that we can recover from this weakness by bridging the gap between sequential adversarial team games and 2-player games. In particular, we propose a new, suitable game representation that we call \emph{team-public-information}, in which a team is represented as a single coordinator who only knows information common to the whole team and prescribes to each member an action for any possible private state. The resulting representation is highly \emph{explainable}, being a 2-player tree in which the team's strategies are behavioral with a direct interpretation and more expressive than the original extensive form when designing abstractions. Furthermore, we prove payoff equivalence of our representation, and we provide techniques that, starting directly from the extensive form, generate dramatically more compact representations without information loss. Finally, we experimentally evaluate our techniques when applied to a standard testbed, comparing their performance with the current state of the art.

==> content/3_tmecor.tex <==
\section{How to Enforce Coordination Between Team Members}\label{sec:tmecor}

When considering ATGs, the problem of computing optimal strategies for the team of agents becomes inherently much more complex than with 2p0s games. 
%
This is basically due to team players' need for coordinating their strategies to maximize their utility. 
%
In practice, such a requirement on coordination is translated into the formulation of an \emph{ad hoc} solution concept for ATGs. 
%
Von Stengel and Koller, in \cite{VonStengelKoller97}, introduce the \emph{Team Maxmin Equilibrium} (TME), which is defined as the NE in which the team's utility is maximized. 
%
The solution concept described by the TME exhibits some appealing characteristics: (i) in some cases it can be arbitrarily more efficient in terms of payoffs for the team with respect to a NE, (ii) it is unique (except for degeneracies), thus it does not suffer from equilibrium selection issues \cite{Basilico2016teammaxmin,Basilico2017ComputingTT,Celli2018ComputationalRF}.
%
However, it is not easy to be computed as it does not admit a convex mathematical formulation \cite{Farina2021ConnectingOE}.

If the coordination of team's strategies is done \emph{ex-ante}\footnote{Note that different forms of coordination are possible, (\emph{e.g.}, intra-play) but they require communication capabilities between the team members that may not be allowed in arbitrary games.} (\emph{i.e.}, before the beginning of each game), a new solution concept can be introduced, called \emph{Team Maxmin Equilibrium with a Correlation device} (TMEcor) \cite{Celli2018ComputationalRF}. 
%
Such coordination has the advantage to increase the expected utility of the team \cite{Celli2018ComputationalRF}. Moreover, differently from what happens with the TME, the TMEcor can be computed through a Linear Program working with joint normal-form plans of the team players: 
%
\begin{equation}\label{eq:tmecor}
\begin{array}{l}\displaystyle
\max_{\mu_\team}\min_{\mu_o} \sum_{z\in\Z}\hspace{.4cm} \mu_\team[z]\,\mu_o[z]\,u_\team(z)\\
\hspace{.3cm}\textnormal{s.t. }\hspace{.5cm}\mu_\team\in\Delta(\bigtimes\limits_{p\in\team}\Pi_p)\\[4mm]
\hspace{1.3cm}\mu_o\in\Delta(\Pi_o).
\end{array}
\end{equation}
% 

In general, the size of the strategy space of the team $\bigtimes_{p\in\team} \Pi_p$ grows exponentially in the number of team members, thus increasing the complexity of solving the LP in Equation~\eqref{eq:tmecor}.
%
There are, however, some specific cases in which we can compute or approximate efficiently the TMEcor, simply by considering all the team members as a unique \emph{meta-player} $\team$ and applying state-of-the-art algorithms for finding NE in 2p0s games.
%
In order to use these techniques, we need that the meta-player has perfect recall. 
%
The requirement of perfect recallness for the team is satisfied only when the information available to the team players is \emph{symmetric}, (\emph{i.e.}, when they all observe an action or none of them does).
%
Unfortunately, this is not usually the case. 
%
In principle, the sources of imperfect recallness for the team can be several\footnote{We refer the interested reader to Appendix~\ref{app:info_structure} for a more detailed description of the aforementioned cases.
}: (i) non-visibility over a team member's actions, (ii) non-visible game structure, (iii) private information disclosed only to a subset of team members.
Mathematical programming algorithms \cite{Celli2018ComputationalRF,Farina2018ExAC,Farina2021ConnectingOE}  address the problem of imperfect recallness for the team by considering the space of joint strategies. When the support of the TMEcor strategy for the team is small, they can efficiently converge to the equilibrium.
%
On the other hand, MARL solutions, like SIMS \cite{Cacciamani2021MultiAgentCI}, are capable of solving case (i), but fail to deal with the other sources of imperfect recallness.
%
In this work, exploiting the concept of \emph{public information}, we introduce a method allowing us to deal with all the three sources of imperfect recallness, thus opening to the possibility of using state-of-the-art RL algorithms (\emph{e.g.}, Deep-CFR\cite{Brown2019DeepCR}) to solve ATGs.
%
We do this first by defining a game formalism that enriches EFGs with information on public observability of actions, and then by formulating a method that casts the original ATG into an equivalent 2p0s EFG. 
\fe{Incorporare in Sezione 2 accorciando}


==> content/6_pruning.tex <==
%\section{Information-lossless Abstractions}
\section{Generating More Concise Representations}
\label{sec:pruning}

As aforementioned, in the worst case, our representation cannot have a size upper bounded by a polynomial in the size of the extensive form unless $\mathsf{P}= \mathsf{NP}$. Nevertheless, in many cases, the game tree generated by our conversion may contain redundant information, and thus it can be compressed without any loss of information. In the following, we provide two different, mutually exclusive, procedures generating a much more concise team-public-information representation of an adversarial team game. 


%\nc{\begin{itemize}
%     \item Capire se i nomi che seguono sono i piu' appropriati oppure possiamo cambiarli.
%    \item Statement formale che dice cosa si puo' fare in versione online.
%    \item Accorpare questa sezione con la successiva. Io prima metterei la discussione generale (quindi la sezione successiva), e poi metterei questa sezione.
%\end{itemize}}

%The conversion procedure presented above allows us to prove the equivalence between the original ATG and its converted version. A crucial question is whether we can produce a reduced, more compact variant of our representation. The main reason is that, indeed, applying Algorithm~\ref{alg:PubTeam} to a public state in the original game with $A$ actions for $S$ possible private states results in $A^S$ prescriptions, producing a tree with an exponentially large fan-out.
% While the computation of a TMECor has an unavoidable exponential complexity due to the \textsf{NP}-hardness of the problem\ma{CITA}, any 2p0s solving algorithm can strongly benefit from any improvement made to the game size. 

%We propose three algorithms, each returning an information-lossless abstraction of the converted game to attenuate the computational burden of the converted game allowing the application of existing algorithms for equilibrium computation or approximation.

\textbf{Pruning procedure}. 
The rationale behind this procedure is the following. Whenever the coordinator  prescribes a team member to play an action $a$ such that $Pub_{\mathcal{P}}(a) = \mathrm{pub}$ where $\mathcal{P}$ is the team, the prescriptions for the private states in the following part of the tree can be separated. Since the number of prescriptions depends on the number of private states, their separation allows a dramatic reduction of the number of prescriptions without any loss of information. 
%
% This pruning effect is particularly effective when the chosen prescriptions are various, suggesting many different actions; on the other hand, uninformative prescriptions associating the same action to all private states do not allow the exclusion of any private state.

The pseudocode of the procedure is provided in Algorithm~\ref{alg:pruned_PubTeam} in Appendix~\ref{app:pruned_PubTeam}. It takes in input the extensive-form game and directly returns in output the pruned representation without the need for generating the game by Algorithm~\ref{alg:PubTeam} and then processing it. In particular, the procedure can be obtained by a simple modification of Algorithm~\ref{alg:PubTeam}, adding a parameter $\mathcal X$ in \algoname{PubTeamConv} which is used to store the private states that can be excluded in the following part of the tree once played a public action. 
By excluding every information set in $\mathcal X$ when building the prescription in Line~\ref{lst:line:prescription}, we can effectively prune the number of private states to be considered by the coordinator.
An example of pruned representation is provided in Fig.~\ref{fig:convPrunedExample} in Appendix~\ref{app:pruned_PubTeam}.
We can state the following.

\begin{restatable}{theorem}{theoremprunedbasic}
Given a public-turn-taking vEFG $\mathcal{G}$, the corresponding TPI $\mathcal G' = \algoname{ConvertGame}(\mathcal G) $ and the pruned version $\mathcal G''$, then $\mathcal G'$ and $\mathcal G''$ are realization-equivalent in the sense that, given any strategy $\pi_t'$ for $\mathcal G'$, then there exists a strategy $\pi_t''$ for $\mathcal G''$ such that $\forall \pi_c, \pi_o$: 
    \begin{equation*}
        u_t' (\pi_t', \pi_o, \pi_c) = u_t'' (\pi_t'', \pi_o, \pi_c).
    \end{equation*}
    The converse is also true.
\fe{Formalizzare il nome della procedura di pruning}
\end{restatable}

\nc{THM: l'albero prodotto e' senza perdita di informazione ... --- probabilmente lo statement deve essere che la forma normale e' la stessa e quindi vale l'equivalenza strategica.}
\lu{idea per proof: se siamo sicuri che una carta non è possible che sia in mano a uno dei giocatori, allora  gli alberi derivanti dal prescrivere azioni diverse per quella carta saranno completamente sovrapponibili (siccome la prescrizione per quella carta non verrà mai eseguita). Quindi possiamo unire diverse prescrizioni perchè gli alberi derivanti sono identici}

Interestingly, when the extensive-form game can be concisely encoded as a finite-state machine so as to avoid the storage of the entire tree, the pruning procedure can be directly applied to the finite-state machine and returns a new finite-state machine that describing the converted game. Thus, we can concisely encode the pruning team-public-information representation. This is particularly important when using MARL techniques. 


\textbf{Folding procedure}. The rationale behind this procedure is the following. 
Consider the case in which the space of the players' signals is interdependent. For example, given a deck of three cards $K,Q,J$, when a player draws $K$, she can safely infer that the other the players cannot draw $K$. In our converted game, we can dramatically reduce the space of the prescriptions without loss of information by forcing a probability equal to zero to all the beliefs that can be excluded as aforementioned. Such a representation is similar to the public belief state representation proposed in \cite{Brown_Bakhtin_Lerer_Gong_2020}. An example of folded representation is provided in Fig.~\ref{fig:convPrunedExample} in Appendix~\ref{app:pruned_PubTeam}. 


%Consider an action of chance that can be observed by some team member, while it cannot be seen by the adversary (\emph{e.g.}, a private card in poker). We can avoid adding this node to the converted game and instead maintain the probability that each player is in a specific private state, given that some may be excluded as done by the pruning procedure. Then, we modify the chance node $h''$ after each prescription to sample an action according to the sum of the probabilities of the private states for which that action has been prescribed.
%In the original game, chance outcomes are explicitly represented independently by the visibility of the outcomes, branching the game tree into different subgames according to the specific outcome. Consider the case of the extraction of a specific outcome when this is private information for a team member and unseen by the adversary. In the converted game, such an outcome is not visible to any player, and can therefore be safely postponed as long as no specific action depends on it. The folding representation takes advantage of this property to avoid sampling these types of private states and instead samples an action from the prescription depending on the probability (also called belief) that at a certain point in the game a specific private state is present given the previous actions of all players. The dummy chance nodes $h''$ instantiated in Algorithm \ref{alg:PubTeam} therefore may present different actions each with a probability that is the sum of the probability of the private states for which that action has been prescribed. This representation also takes advantage of the computed beliefs to reduce the prescriptions given by the coordinator as in the pruning representation.
%
%Overall, the game size is reduced in case many private states for the players are sampled. 
%Such a representation is similar to the public belief state representation proposed in \cite{Brown_Bakhtin_Lerer_Gong_2020}. The name folding representation derives from the fact that trajectories with the same public actions but different private states are folded one over the other in the converted game.

%The pseudocode is provided in ... \nc{come cambia il codice???} An example of representation generated by procedure YYY is provided in YYY in Appendix ... We can state the following.

%\nc{THM: l'albero prodotto e' senza perdita di informazion ... --- probabilmente lo statement deve essere che la forma normale e' la stessa e quindi vale l'equivalenza strategica.}




%\textbf{Safe Imperfect Recallness}. Whenever a team player is in a state with three or more actions available, a specific action is played and some possible private states are excluded from the belief. The specific actions prescribed for the excluded states are not important to describe the information state of the player; we can therefore forget part of the prescription and have imperfect recall among different prescriptions with different prescribed actions for excluded states. While this abstraction technique does not directly reduce the number of nodes, it reduces the number of information sets, simplifying the information structure of the game.  This reduces the space requirements to represent the strategies and makes the algorithms converge faster. This abstraction technique is theoretically sound, and the convergence properties of CFR in this imperfect-recall setting have already been addressed by \cite{Lanctot_Gibson_Burch_Zinkevich_Bowling_2012}. Examples of the application of the techniques described above are shown in Appendix~\ref{app:figures}. 

==> content/7_expressivity.tex <==
\section{Abstractions and Adversarial Team Games}
\label{sec:expressivity}

Abstractions demonstrated a successful tool to tackle real-world 2p0s games. Customarily, abstractions are obtained by merging different infosets of the same player (called \emph{state} abstractions) and/or different actions of the same player at the same infoset (called \emph{action} abstractions). To the best of our knowledge, abstractions in ATGs are unexplored so far. Our team-public-information representation provides a suitable and direct tool over which we can define abstractions for ATGs as the team's strategies are behavioral. In particular, we show that the extensive-form representation is not sufficiently expressive when designing abstractions for ATGs. We can state the following.

\begin{restatable}{proposition}{propos} Any action or state abstraction that, once applied to an extensive-form game $\mathcal{G}$, returns a perfect-recall timeable game can be mapped specularly in the team-public-information representation $\mathcal{G}' = \algoname{ConvertGame} (\mathcal{G})$. The reverse is not true.
\label{th:prop_abs}
\end{restatable}
It can be easily observed that the properties required by the above proposition are satisfied by the most abstractions, \emph{e.g.}, \cite{10.1145/1284320.1284324,DBLP:conf/aaai/GilpinSS07}.


%propos
%In the case of abstractions generating games with imperfect recall, we can state the following.

%\nc{PROP: scrivere una proposizione qui per il caso a imperfect recall}

%\nc{dire che (sperabilmente) tutte le astrazioni note soddisfano le condizioni sopra: game srink, imperfect recall di lanctot, card binning}
%Proposition~\ref{th:prop_abs} shows that the converted game is able to encode more information than the original game, suggesting that this higher expressive power could be used to design specific abstraction techniques that also work with the space of players' strategies.





%In this section, we compare the expressiveness of our converted game w.r.t. to the original extensive-form representation.

%While adversary and chance players have an identical information structure as in the original game, the converted game presents a richer information structure for what concerns the team players. 
%
%The use of a shared coordinator strategy allows the players to know the exact action played by their teammates for any of their private information states. This is similar to performing an \textit{inflation} \cite{Kaneko1995BehaviorSM} on the original game, recovering the extra information given to the players thanks to the property that, through \emph{ex-ante} coordination, they know the action played by their teammates in each information set.

%Our converted game serves the same purpose as the \textit{Auxiliary game} introduced in \cite{Farina2018ExAC}. The goal is the same: explicitly representing the initial coordination between team members to address the imperfect recallness when representing the team as a unique player. 
%
%However, in our case, the coordinator gives local prescriptions instead of the complete \emph{ex-ante} plan coordination of \cite{Farina2018ExAC}. 
%
%This approach has multiple advantages:
%\begin{itemize}
%    \item the extensive-form representation is more efficient than the normal form with respect to the size of the resulting game \cite{Stengel1997ComputingNF}. Our converted representation takes advantage of this issue and resulting in the use of a more tractable game tree if compared to the one obtained from the normal form coordination proposed in \cite{Farina2018ExAC};
    %
%    \item the sequential structure of coordination in our converted game allows the use of the abstraction techniques, as described in Section~\ref{sec:pruning};
    %
%    \item our conversion maintains the structure of the original game. This results in a more interpretable tree structure, which is crucial for the design of abstraction techniques;
    %
%    \item the auxiliary game of \cite{Farina2018ExAC} uses an initial coordination node with an action for each joint normal-form plan of all team members but one. Instead, our converted game presents nodes with a smaller fanout, thanks to the localized coordination. This makes it feasible to apply \textit{subgame solving} techniques, which proved crucial for the good performance of scalable techniques.
%\end{itemize}
%
% Overall, the efficiency enhancements allow us to work in the full converted game, without resorting to \textit{column generation} techniques. The opportunities opened for the use of abstractions and 

% This different expressive power has direct implications on the effect of applying an abstraction \lu{inserire cit} technique.

%We can also compare the expressive power of our public-turn-making representation with the original extensive form by considering the effect of (information-lossless/loss) abstractions.
